How to Make Your Approximation Algorithm Private: A Black-Box Differentially-Private Transformation for Tunable Approximation Algorithms of Functions with Low Sensitivity

We develop a framework for efficiently transforming certain approximation algorithms into differentially-private variants, in a black-box manner. Specifically, our results focus on algorithms A that output an approximation to a function f of the form $(1-a)f(x)-k \leq A(x) \leq (1+a)f(x)+k$, where $k \in \mathbb{R}_{\geq 0}$ denotes additive error and $a \in [0,1)$ denotes multiplicative error can be``tuned" to small-enough values while incurring only a polynomial blowup in the running time/space. We show that such algorithms can be made DP without sacrificing accuracy, as long as the function f has small global sensitivity. We achieve these results by applying the smooth sensitivity framework developed by Nissim, Raskhodnikova, and Smith (STOC 2007). Our framework naturally applies to transform non-private FPRAS and FPTAS algorithms into $\epsilon$-DP approximation algorithms where the former case requires an additional postprocessing step. We apply our framework in the context of sublinear-time and sublinear-space algorithms, while preserving the nature of the algorithm in meaningful ranges of the parameters. Our results include the first (to the best of our knowledge) $\epsilon$-edge DP sublinear-time algorithm for estimating the number of triangles, the number of connected components, and the weight of a minimum spanning tree of a graph. In the area of streaming algorithms, our results include $\epsilon$-DP algorithms for estimating Lp-norms, distinct elements, and weighted minimum spanning tree for both insertion-only and turnstile streams. Our transformation also provides a private version of the smooth histogram framework, which is commonly used for converting streaming algorithms into sliding window variants, and achieves a multiplicative approximation to many problems, such as estimating Lp-norms, distinct elements, and the length of the longest increasing subsequence.

==> otherapplications.tex <==

\section{Other Applications}

\paragraph{Knapsack Problem. }Given a knapsack of size $B \in \mathbb{Z}^+$, and a set $S=\{a_1, \ldots,a_n\}$ of objects with corresponding sizes $s(a_i) \in \mathbb{Z}^+$ and profits $p(a_i) \in \mathbb{Z}^+$. The goal is to find the optimal subset of objects whose total size is bounded by $B$ and has the maximum possible total profit. We consider neighboring input sets $S \sim S'$ as follows: there exists $1 \leq i^* \leq n$ such that $s(a_{i^*})=s(a'_{i^*})-1$. Thus the global sensitivity of this problem is 1. \jeremiah{Maybe discuss that another natural version would have high sensitivity and discuss this as limintation of our techniques i.e., we do require low global sensitivity...} \jeremiah{Put in appendix? Maybe mention after FTPAS section?}
\begin{corollary}
Suppose $\calA$ is an FPTAS for the knapsack problem and runs in time $\O{n^2 \lfloor\frac{n}{\alpha} \rfloor}$. Then for all $\eps > 0$, there exists an algorithm $\calA'$ that runs in time $\O{n^2 \lfloor\frac{n \log(n)}{\eps \alpha} \rfloor}$ such that  
\begin{enumerate}
    \item (Privacy) $\calA'$ is $\eps$-differentially private. %where $\eps$ is constant.% and $\delta=\frac{1}{n^c}$
    \item (Accuracy) For all $D \in \calD^n$, we have that with probability $\geq 9/10$,
    $$(1-\alpha')f(D) -  \frac{C}{\eps} \leq \calA'_f(D) \leq (1+\alpha')f(D) + \frac{C}{\eps}$$
    where $\alpha'=\frac{\alpha (\eps+C)}{100 \log n}$ for some constant $C>7$. %, and $\Delta_f:=\max_{D,D'\in\calD^n,D \sim D'}\|f(D)-f(D')\|_1. $
\end{enumerate}
\end{corollary}

\jeremiah{Eliminate if no results here...}
\paragraph{Network Unreliability}
Given a graph $G$ and a failure probability $p$, we want to compute the probability $\mu_G(p)$ that $G$ becomes disconnected when edges fail independently with probability $p$~\cite{Karger17}. For edge neighboring graphs $G\sim_e G'$, suppose the failure probability is $p$ for the edges of both graphs. Then the global sensitivity of $\mu_G(p) = p$.    \tanote{can we assume that the probability of failure for edges is fixed over neighboring graphs? } 

\paragraph{Approximating TVD for product distributions} 
\samson{Can we formally define the problem/model?}
\begin{theorem}~\cite{FGJW22}
Let $[q]= \{1,2,\ldots, q\}$ be a finite set. There exists an algorithm such that given two product distributions $P,Q$ over $[q]^n$ and parameters $\alpha>0$ and $0 < \gamma< 1$, it outputs a random value $\hat{d}$ in time $O\left(\frac{n^3}{\log(1/\gamma)}\right)$ such that $(1-\alpha) d_{TV}(P,Q) \leq \hat{d} \leq (1+\alpha)d_{TV}(P,Q)$ holds with probability at least $1-\gamma$.
\end{theorem}
The algorithm can handle the case where each coordinate has a different domain size without any change. The input product distributions are given by the marginal probability for each coordinate and each $c \in [q]$ in binary. The stated running time assumes that all arithmetic oprations can be done in $O(1)$ time. 
\tanote{The input to this FPRAS is two product distributions... how we do we define neighboring distributions? If they differ by a coordinate?}

\tanote{include knapsack where the value of an item can change by 1, if we define neighboring as addition or deletion of an item then this has high sensitivity }
